Augmenting deep neural networks with symbolic knowledge: Towards trustworthy and interpretable AI for education

Artificial neural networks (ANNs) have shown to be amongst the most important artificial intelligence (AI) techniques in educational applications, providing adaptive educational services. However, their educational potential is limited in practice due to three major challenges: i) difficulty in incorporating symbolic educational knowledge (e.g., causal relationships, and practitioners' knowledge) in their development, ii) learning and reflecting biases, and iii) lack of interpretability. Given the high-risk nature of education, the integration of educational knowledge into ANNs becomes crucial for developing AI applications that adhere to essential educational restrictions, and provide interpretability over the predictions. This research argues that the neural-symbolic family of AI has the potential to address the named challenges. To this end, it adapts a neural-symbolic AI framework and accordingly develops an approach called NSAI, that injects and extracts educational knowledge into and from deep neural networks, for modelling learners computational thinking. Our findings reveal that the NSAI approach has better generalizability compared to deep neural networks trained merely on training data, as well as training data augmented by SMOTE and autoencoder methods. More importantly, unlike the other models, the NSAI approach prioritises robust representations that capture causal relationships between input features and output labels, ensuring safety in learning to avoid spurious correlations and control biases in training data. Furthermore, the NSAI approach enables the extraction of rules from the learned network, facilitating interpretation and reasoning about the path to predictions, as well as refining the initial educational knowledge. These findings imply that neural-symbolic AI can overcome the limitations of ANNs in education, enabling trustworthy and interpretable applications.

==> references.tex <==
@article{vincent2020trustworthy,
  title={Trustworthy artificial intelligence (AI) in education: Promises and challenges},
  author={Vincent-Lancrin, St{\'e}phan and Van der Vlies, Reyer},
  journal={OECD},
  year={2020},
  publisher={OECD}
}
@article{conati20238,
  title={8. Student modeling in open-ended learning environments},
  author={Conati, Cristina and Lall{\'e}, S{\'e}bastien},
  journal={Handbook of Artificial Intelligence in Education},
  pages={170--183},
  year={2023},
  publisher={Edward Elgar Publishing}
}
@article{hooshyar2019systematic,
  title={A systematic review of data-driven approaches in player modeling of educational games},
  author={Hooshyar, Danial and Yousefi, Moslem and Lim, Heuiseok},
  journal={Artificial Intelligence Review},
  volume={52},
  pages={1997--2017},
  year={2019},
  publisher={Springer}
}
@article{abyaa2019learner,
  title={Learner modelling: systematic review of the literature from the last 5 years},
  author={Abyaa, Abir and Khalidi Idrissi, Mohammed and Bennani, Samir},
  journal={Educational Technology Research and Development},
  volume={67},
  pages={1105--1143},
  year={2019},
  publisher={Springer}
}
@article{garcez2022neural,
  title={Neural-symbolic learning and reasoning: A survey and interpretation},
  author={Garcez, Artur d’Avila and Bader, Sebastian and Bowman, Howard and Lamb, Luis C and de Penning, Leo and Illuminoo, BV and Poon, Hoifung and Zaverucha, COPPE Gerson},
  journal={Neuro-Symbolic Artificial Intelligence: The State of the Art},
  volume={342},
  number={1},
  pages={327},
  year={2022},
  publisher={IOS Press}
}
@article{lenat1985cyc,
  title={CYC: Using common sense knowledge to overcome brittleness and knowledge acquisition bottlenecks},
  author={Lenat, Douglas B and Prakash, Mayank and Shepherd, Mary},
  journal={AI magazine},
  volume={6},
  number={4},
  pages={65--65},
  year={1985}
}
@inproceedings{bhanuse2021systematic,
  title={A systematic review: deep learning based e-learning recommendation system},
  author={Bhanuse, Roshan and Mal, Sandip},
  booktitle={2021 International Conference on Artificial Intelligence and Smart Systems (ICAIS)},
  pages={190--197},
  year={2021},
  organization={IEEE}
}
@article{hernandez2019systematic,
  title={A systematic review of deep learning approaches to educational data mining},
  author={Hern{\'a}ndez-Blanco, Antonio and Herrera-Flores, Boris and Tom{\'a}s, David and Navarro-Colorado, Borja and others},
  journal={Complexity},
  volume={2019},
  year={2019},
  publisher={Hindawi}
}
@article{hooshyar2022gamedkt,
  title={GameDKT: Deep knowledge tracing in educational games},
  author={Hooshyar, Danial and Huang, Yueh-Min and Yang, Yeongwook},
  journal={Expert Systems with Applications},
  volume={196},
  pages={116670},
  year={2022},
  publisher={Elsevier}
}
@article{piech2015deep,
  title={Deep knowledge tracing},
  author={Piech, Chris and Bassen, Jonathan and Huang, Jonathan and Ganguli, Surya and Sahami, Mehran and Guibas, Leonidas J and Sohl-Dickstein, Jascha},
  journal={Advances in neural information processing systems},
  volume={28},
  year={2015}
}
@inproceedings{torralba2011unbiased,
  title={Unbiased look at dataset bias},
  author={Torralba, Antonio and Efros, Alexei A},
  booktitle={CVPR 2011},
  pages={1521--1528},
  year={2011},
  organization={IEEE}
}
@inproceedings{agrawal2018don,
  title={Don't just assume; look and answer: Overcoming priors for visual question answering},
  author={Agrawal, Aishwarya and Batra, Dhruv and Parikh, Devi and Kembhavi, Aniruddha},
  booktitle={Proceedings of the IEEE conference on computer vision and pattern recognition},
  pages={4971--4980},
  year={2018}
}
@article{gretton2010consistent,
  title={Consistent nonparametric tests of independence},
  author={Gretton, Arthur and Gy{\"o}rfi, L{\'a}szl{\'o}},
  journal={The Journal of Machine Learning Research},
  volume={11},
  pages={1391--1423},
  year={2010},
  publisher={JMLR. org}
}
@article{srivastava2023addressing,
  title={Addressing Spurious Correlations in Machine Learning Models: A Comprehensive Review},
  author={Srivastava, Mashrin},
  journal={OSF Preprints},
  year={2023},
  publisher={OSF Preprints}
}
@article{zech2018variable,
  title={Variable generalization performance of a deep learning model to detect pneumonia in chest radiographs: a cross-sectional study},
  author={Zech, John R and Badgeley, Marcus A and Liu, Manway and Costa, Anthony B and Titano, Joseph J and Oermann, Eric Karl},
  journal={PLoS medicine},
  volume={15},
  number={11},
  pages={e1002683},
  year={2018},
  publisher={Public Library of Science San Francisco, CA USA}
}
@misc{unesco2019beijing,
  title={Beijing consensus on artificial intelligence and education},
  author={UNESCO},
  year={2019},
  publisher={Unesco Paris}
}
@article{conati2018ai,
  title={AI in Education needs interpretable machine learning: Lessons from Open Learner Modelling},
  author={Conati, Cristina and Porayska-Pomsta, Kaska and Mavrikis, Manolis},
  journal={arXiv preprint arXiv:1807.00154},
  year={2018}
}
@article{meltzer2022european,
  title={The European Union AI Act: Next steps and issues for building international cooperation in AI},
  author={Meltzer, Joshua P and Tielemans, Aaron},
  journal={Brookings Institution},
  year={2022},
  publisher={Brookings Institution}
}
@article{hooshyar2022three,
  title={A Three-Layered Student Learning Model for Prediction of Failure Risk in Online Learning},
  author={Hooshyar, Danial and Huang, Yueh-Min and Yang, Yeongwook and others},
  journal={Human-centric Computing and Information Sciences},
  volume={12},
  year={2022},
  publisher={Korea Information Processing Society}
}
@article{saarela2021explainable,
  title={Explainable student agency analytics},
  author={Saarela, Mirka and Heilala, Ville and J{\"a}{\"a}skel{\"a}, P{\"a}ivikki and Rantakaulio, Anne and K{\"a}rkk{\"a}inen, Tommi},
  journal={IEEE Access},
  volume={9},
  pages={137444--137459},
  year={2021},
  publisher={IEEE}
}
@inproceedings{lakkaraju2020fool,
  title={" How do I fool you?" Manipulating User Trust via Misleading Black Box Explanations},
  author={Lakkaraju, Himabindu and Bastani, Osbert},
  booktitle={Proceedings of the AAAI/ACM Conference on AI, Ethics, and Society},
  pages={79--85},
  year={2020}
}
@inproceedings{slack2020fooling,
  title={Fooling lime and shap: Adversarial attacks on post hoc explanation methods},
  author={Slack, Dylan and Hilgard, Sophie and Jia, Emily and Singh, Sameer and Lakkaraju, Himabindu},
  booktitle={Proceedings of the AAAI/ACM Conference on AI, Ethics, and Society},
  pages={180--186},
  year={2020}
}
@article{garcez2023neurosymbolic,
  title={Neurosymbolic AI: The 3 rd wave},
  author={Garcez, Artur d’Avila and Lamb, Luis C},
  journal={Artificial Intelligence Review},
  pages={1--20},
  year={2023},
  publisher={Springer}
}
@article{hooshyar2021neural,
  title={Neural-symbolic computing: A step toward interpretable AI in Education},
  author={Hooshyar, Danial and Yang, Yeongwook},
  journal={Bulletin of the Technical Committee on Learning Technology (ISSN: 2306-0212)},
  volume={21},
  number={4},
  pages={2--6},
  year={2021}
}
@article{sarker2021neuro,
  title={Neuro-symbolic artificial intelligence},
  author={Sarker, Md Kamruzzaman and Zhou, Lu and Eberhart, Aaron and Hitzler, Pascal},
  journal={AI Communications},
  volume={34},
  number={3},
  pages={197--209},
  year={2021},
  publisher={IOS Press}
}
@article{chawla2002smote,
  title={SMOTE: synthetic minority over-sampling technique},
  author={Chawla, Nitesh V and Bowyer, Kevin W and Hall, Lawrence O and Kegelmeyer, W Philip},
  journal={Journal of artificial intelligence research},
  volume={16},
  pages={321--357},
  year={2002}
}
@article{kingma2019introduction,
  title={An introduction to variational autoencoders},
  author={Kingma, Diederik P and Welling, Max and others},
  journal={Foundations and Trends{\textregistered} in Machine Learning},
  volume={12},
  number={4},
  pages={307--392},
  year={2019},
  publisher={Now Publishers, Inc.}
}
@book{yegnanarayana2009artificial,
  title={Artificial neural networks},
  author={Yegnanarayana, Bayya},
  year={2009},
  publisher={PHI Learning Pvt. Ltd.}
}
@article{abiodun2018state,
  title={State-of-the-art in artificial neural network applications: A survey},
  author={Abiodun, Oludare Isaac and Jantan, Aman and Omolara, Abiodun Esther and Dada, Kemi Victoria and Mohamed, Nachaat AbdElatif and Arshad, Humaira},
  journal={Heliyon},
  volume={4},
  number={11},
  year={2018},
  publisher={Elsevier}
}
@article{bendangnuksung2018students,
  title={Students’ performance prediction using deep neural network},
  author={Bendangnuksung, Prabu P},
  journal={International Journal of Applied Engineering Research},
  volume={13},
  number={2},
  pages={1171--1176},
  year={2018}
}
@inproceedings{wang2017deep,
  title={Deep knowledge tracing on programming exercises},
  author={Wang, Lisa and Sy, Angela and Liu, Larry and Piech, Chris},
  booktitle={Proceedings of the fourth (2017) ACM conference on learning@ scale},
  pages={201--204},
  year={2017}
}
@inproceedings{fei2015temporal,
  title={Temporal models for predicting student dropout in massive open online courses},
  author={Fei, Mi and Yeung, Dit-Yan},
  booktitle={2015 IEEE international conference on data mining workshop (ICDMW)},
  pages={256--263},
  year={2015},
  organization={IEEE}
}
@inproceedings{teruel2018co,
  title={Co-embeddings for student modeling in virtual learning environments},
  author={Teruel, Milagro and Alonso Alemany, Laura},
  booktitle={Proceedings of the 26th Conference on User Modeling, Adaptation and Personalization},
  pages={73--80},
  year={2018}
}
@article{whitehill2017delving,
  title={Delving deeper into MOOC student dropout prediction},
  author={Whitehill, Jacob and Mohan, Kiran and Seaton, Daniel and Rosen, Yigal and Tingley, Dustin},
  journal={arXiv preprint arXiv:1702.06404},
  year={2017}
}
@inproceedings{abhinav2018lecore,
  title={LeCoRe: A Framework for Modeling Learner's preference.},
  author={Abhinav, Kumar and Subramanian, Venkatesh and Dubey, Alpana and Bhat, Padmaraj and Venkat, Aditya Divakaruni},
  booktitle={EDM},
  year={2018}
}
@inproceedings{wong2018sequence,
  title={Sequence based course recommender for personalized curriculum planning},
  author={Wong, Chris},
  booktitle={Artificial Intelligence in Education: 19th International Conference, AIED 2018, London, UK, June 27--30, 2018, Proceedings, Part II 19},
  pages={531--534},
  year={2018},
  organization={Springer}
}
@article{hooshyar2021predicting,
  title={Predicting course grade through comprehensive modelling of students’ learning behavioral pattern},
  author={Hooshyar, Danial and Yang, Yeongwook},
  journal={Complexity},
  volume={2021},
  pages={1--12},
  year={2021},
  publisher={Hindawi Limited}
}
@inproceedings{taghipour2016neural,
  title={A neural approach to automated essay scoring},
  author={Taghipour, Kaveh and Ng, Hwee Tou},
  booktitle={Proceedings of the 2016 conference on empirical methods in natural language processing},
  pages={1882--1891},
  year={2016}
}
@inproceedings{zhao2017memory,
  title={A memory-augmented neural model for automated grading},
  author={Zhao, Siyuan and Zhang, Yaqiong and Xiong, Xiaolu and Botelho, Anthony and Heffernan, Neil},
  booktitle={Proceedings of the fourth (2017) ACM conference on learning@ scale},
  pages={189--192},
  year={2017}
}
@article{mao2018deep,
  title={Deep Learning vs. Bayesian Knowledge Tracing: Student Models for Interventions.},
  author={Mao, Ye},
  journal={Journal of educational data mining},
  volume={10},
  number={2},
  year={2018}
}
@inproceedings{tang2016deep,
  title={Deep neural networks and how they apply to sequential education data},
  author={Tang, Steven and Peterson, Joshua C and Pardos, Zachary A},
  booktitle={Proceedings of the third (2016) acm conference on learning@ scale},
  pages={321--324},
  year={2016}
}
@article{sharada2018modeling,
  title={Modeling student knowledge retention using deep learning and random forests},
  author={Sharada, N and Shashi, M and Xiong, X},
  journal={Journal of Engineering and Applied Sciences},
  volume={13},
  number={6},
  pages={1347--1353},
  year={2018}
}
@inproceedings{alam2018reduced,
  title={A reduced feature based neural network approach to classify the category of students},
  author={Alam, Mirza Mohtashim and Mohiuddin, Karishma and Das, Amit Kishor and Islam, Md Kabirul and Kaonain, Md Shamsul and Ali, Md Haider},
  booktitle={Proceedings of the 2nd International Conference on Innovation in Artificial Intelligence},
  pages={28--32},
  year={2018}
}
@article{kim2018gritnet,
  title={GritNet: Student performance prediction with deep learning},
  author={Kim, Byung-Hak and Vizitei, Ethan and Ganapathi, Varun},
  journal={arXiv preprint arXiv:1804.07405},
  year={2018}
}
@article{tato2017convolutional,
  title={Convolutional Neural Network for Automatic Detection of Sociomoral Reasoning Level.},
  author={Tato, Ange and Nkambou, Roger and Dufresne, Aude and Beauchamp, Miriam H},
  journal={International Educational Data Mining Society},
  year={2017},
  publisher={ERIC}
}
@article{min2016predicting,
  title={Predicting Dialogue Acts for Intelligent Virtual Agents with Multimodal Student Interaction Data.},
  author={Min, Wookhee and Wiggins, Joseph B and Pezzullo, Lydia G and Vail, Alexandria K and Boyer, Kristy Elizabeth and Mott, Bradford W and Frankosky, Megan H and Wiebe, Eric N and Lester, James C},
  journal={International Educational Data Mining Society},
  year={2016},
  publisher={ERIC}
}
@article{sharma2016livelinet,
  title={LIVELINET: A Multimodal Deep Recurrent Neural Network to Predict Liveliness in Educational Videos.},
  author={Sharma, Arjun and Biswas, Arijit and Gandhi, Ankit and Patil, Sonal and Deshmukh, Om},
  journal={International Educational Data Mining Society},
  year={2016},
  publisher={ERIC}
}
@article{besold2017d,
  title={A. d. Garcez, S. Bader, H. Bowman, P. Domingos, P. Hitzler, K.-U. K{\"u}hnberger, LC Lamb, D. Lowd, PMV Lima et al.,“Neural-symbolic learning and reasoning: A survey and interpretation,”},
  author={Besold, TR},
  journal={arXiv preprint arXiv:1711.03902},
  year={2017}
}
@article{tran2016deep,
  title={Deep logic networks: Inserting and extracting knowledge from deep belief networks},
  author={Tran, Son N and Garcez, Artur S d’Avila},
  journal={IEEE transactions on neural networks and learning systems},
  volume={29},
  number={2},
  pages={246--258},
  year={2016},
  publisher={IEEE}
}
@article{hu2016harnessing,
  title={Harnessing deep neural networks with logic rules},
  author={Hu, Zhiting and Ma, Xuezhe and Liu, Zhengzhong and Hovy, Eduard and Xing, Eric},
  journal={arXiv preprint arXiv:1603.06318},
  year={2016}
}
@inproceedings{serafini2016learning,
  title={Learning and reasoning with logic tensor networks},
  author={Serafini, Luciano and d’Avila Garcez, Artur S},
  booktitle={Conference of the Italian Association for Artificial Intelligence},
  pages={334--348},
  year={2016},
  organization={Springer}
}
@article{li2019augmenting,
  title={Augmenting neural networks with first-order logic},
  author={Li, Tao and Srikumar, Vivek},
  journal={arXiv preprint arXiv:1906.06298},
  year={2019}
}
@article{shakya2021student,
  title={Student Strategy Prediction Using a Neuro-Symbolic Approach.},
  author={Shakya, Anup and Rus, Vasile and Venugopal, Deepak},
  journal={International Educational Data Mining Society},
  year={2021},
  publisher={ERIC}
}
@inproceedings{muralidhar2018incorporating,
  title={Incorporating prior domain knowledge into deep neural networks},
  author={Muralidhar, Nikhil and Islam, Mohammad Raihanul and Marwah, Manish and Karpatne, Anuj and Ramakrishnan, Naren},
  booktitle={2018 IEEE international conference on big data (big data)},
  pages={36--45},
  year={2018},
  organization={IEEE}
}
@inproceedings{hooshyar2019autothinking,
  title={AutoThinking: An adaptive computational thinking game},
  author={Hooshyar, Danial and Lim, Heuiseok and Pedaste, Margus and Yang, Kisu and Fathi, Moein and Yang, Yeongwook},
  booktitle={Innovative Technologies and Learning: Second International Conference, ICITL 2019, Troms{\o}, Norway, December 2--5, 2019, Proceedings 2},
  pages={381--391},
  year={2019},
  organization={Springer}
}
@article{hooshyar2021gaming,
  title={From gaming to computational thinking: An adaptive educational computer game-based learning approach},
  author={Hooshyar, Danial and Pedaste, Margus and Yang, Yeongwook and Malva, Liina and Hwang, Gwo-Jen and Wang, Minhong and Lim, Heuiseok and Delev, Dejan},
  journal={Journal of Educational Computing Research},
  volume={59},
  number={3},
  pages={383--409},
  year={2021},
  publisher={SAGE Publications Sage CA: Los Angeles, CA}
}
@article{towell1994knowledge,
  title={Knowledge-based artificial neural networks},
  author={Towell, Geoffrey G and Shavlik, Jude W},
  journal={Artificial intelligence},
  volume={70},
  number={1-2},
  pages={119--165},
  year={1994},
  publisher={Elsevier}
}
@article{ribeiro2016model,
  title={Model-agnostic interpretability of machine learning},
  author={Ribeiro, Marco Tulio and Singh, Sameer and Guestrin, Carlos},
  journal={arXiv preprint arXiv:1606.05386},
  year={2016}
}
@article{azevedo201410,
  title={10 Metacognition in Multimedia Learning},
  author={AZEVEDO, ROGER and DEVER, DARYN},
  journal={The Cambridge Handbook of Multimedia Learning},
  year={2014}
}
@article{greene2009macro,
  title={A macro-level analysis of SRL processes and their relations to the acquisition of a sophisticated mental model of a complex system},
  author={Greene, Jeffrey Alan and Azevedo, Roger},
  journal={Contemporary educational psychology},
  volume={34},
  number={1},
  pages={18--29},
  year={2009},
  publisher={Elsevier}
}
@article{pekrun2006control,
  title={The control-value theory of achievement emotions: Assumptions, corollaries, and implications for educational research and practice},
  author={Pekrun, Reinhard},
  journal={Educational psychology review},
  volume={18},
  pages={315--341},
  year={2006},
  publisher={Springer}
}
@incollection{Winne2022,
  doi = {10.1017/9781108888295.007},
  url = {https://doi.org/10.1017/9781108888295.007},
  year = {2022},
  month = apr,
  publisher = {Cambridge University Press},
  pages = {93--113},
  author = {Philip H. Winne and Roger Azevedo},
  title = {Metacognition and Self-Regulated Learning},
  booktitle = {The Cambridge Handbook of the Learning Sciences}
}
@inproceedings{el2020investigating,
  title={Investigating the Learning Impact of Autothinking Educational Game on Adults: A Case Study of France.},
  author={El Mawas, Nour and Hooshyar, Danial and Yang, Yeongwook},
  booktitle={CSEDU (2)},
  pages={188--196},
  year={2020}
}
@article{hooshyar2022effects,
  title={Effects of technology-enhanced learning approaches on learners with different prior learning attitudes and knowledge in computational thinking},
  author={Hooshyar, Danial},
  journal={Computer Applications in Engineering Education},
  volume={30},
  number={1},
  pages={64--76},
  year={2022},
  publisher={Wiley Online Library}
}
@misc{europaBiasAlgorithms,
	author = {},
	title = {{B}ias in algorithms - {A}rtificial intelligence and discrimination --- fra.europa.eu},
	howpublished = {\url{https://fra.europa.eu/en/publication/2022/bias-algorithm}},
	year = {},
	note = {[Accessed 28-10-2023]},
}
@article{blodgett2020language,
  title={Language (technology) is power: A critical survey of" bias" in nlp},
  author={Blodgett, Su Lin and Barocas, Solon and Daum{\'e} III, Hal and Wallach, Hanna},
  journal={arXiv preprint arXiv:2005.14050},
  year={2020}
}
@article{johnson2019survey,
  title={Survey on deep learning with class imbalance},
  author={Johnson, Justin M and Khoshgoftaar, Taghi M},
  journal={Journal of Big Data},
  volume={6},
  number={1},
  pages={1--54},
  year={2019},
  publisher={Springer}
}
@inproceedings{liusie2022analyzing,
  title={Analyzing biases to spurious correlations in text classification tasks},
  author={Liusie, Adian and Raina, Vatsal and Raina, Vyas and Gales, Mark},
  booktitle={Proceedings of the 2nd Conference of the Asia-Pacific Chapter of the Association for Computational Linguistics and the 12th International Joint Conference on Natural Language Processing},
  pages={78--84},
  year={2022}
}
@article{hooshyar2023modeling,
  title={Modeling Learners to Early Predict Their Performance in Educational Computer Games},
  author={Hooshyar, Danial and El Mawas, Nour and Milrad, Marcelo and Yang, Yeongwook},
  journal={IEEE Access},
  volume={11},
  pages={20399--20417},
  year={2023},
  publisher={IEEE}
}
@inproceedings{venugopal2021neuro,
  title={Neuro-Symbolic Models: A Scalable, Explainable Framework for Strategy Discovery from Big Edu-Data},
  author={Venugopal, Deepak and Rus, Vasile and Shakya, Anup},
  booktitle={Proceedings of the 2nd Learner Data Institute Workshop in Conjunction with The 14th International Educational Data Mining Conference},
  year={2021}
}
@article{ramezankhani2016impact,
  title={The impact of oversampling with SMOTE on the performance of 3 classifiers in prediction of type 2 diabetes},
  author={Ramezankhani, Azra and Pournik, Omid and Shahrabi, Jamal and Azizi, Fereidoun and Hadaegh, Farzad and Khalili, Davood},
  journal={Medical decision making},
  volume={36},
  number={1},
  pages={137--144},
  year={2016},
  publisher={SAGE Publications Sage CA: Los Angeles, CA}
}
@inproceedings{zhou2021examining,
  title={Examining and combating spurious features under distribution shift},
  author={Zhou, Chunting and Ma, Xuezhe and Michel, Paul and Neubig, Graham},
  booktitle={International Conference on Machine Learning},
  pages={12857--12867},
  year={2021},
  organization={PMLR}
}
@article{hutt2019evaluating,
  title={Evaluating Fairness and Generalizability in Models Predicting On-Time Graduation from College Applications.},
  author={Hutt, Stephen and Gardner, Margo and Duckworth, Angela L and D'Mello, Sidney K},
  journal={International Educational Data Mining Society},
  year={2019},
  publisher={ERIC}
}
@article{fiok2022explainable,
  title={Explainable artificial intelligence for education and training},
  author={Fiok, Krzysztof and Farahani, Farzad V and Karwowski, Waldemar and Ahram, Tareq},
  journal={The Journal of Defense Modeling and Simulation},
  volume={19},
  number={2},
  pages={133--144},
  year={2022},
  publisher={SAGE Publications Sage UK: London, England}
}


